AltCLIP: Altering the Language Encoder in CLIP for Extended Language Capabilities

In this work, we present a conceptually simple and effective method to train a strong bilingual/multilingual multimodal representation model. Starting from the pre-trained multimodal representation model CLIP released by OpenAI, we altered its text encoder with a pre-trained multilingual text encoder XLM-R, and aligned both languages and image representations by a two-stage training schema consisting of teacher learning and contrastive learning. We validate our method through evaluations of a wide range of tasks. We set new state-of-the-art performances on a bunch of tasks including ImageNet-CN, Flicker30k-CN, COCO-CN and XTD. Further, we obtain very close performances with CLIP on almost all tasks, suggesting that one can simply alter the text encoder in CLIP for extended capabilities such as multilingual understanding. Our models and code are available at https://github.com/FlagAI-Open/FlagAI.

==> Bilingual CLIP draft/1_introduction.tex <==
\section{Introduction}
Learning a good representation in a joint space for vision and language has been a long pursuit in the research of Artificial Intelligence (AI). Recently, the milestone work of CLIP \cite{radford2021learning} from OpenAI demonstrated impressive zero-shot performances across a number of tasks such as image classification on ImageNet~\cite{deng2009imagenet}, Image-to-Text and Text-to-Image retrieval on Flicker-30k ~\cite{young2014image} and MSCOCO\cite{lin2014microsoft, chen2015microsoft}. There has been the pursuit of building contrastive language-image models in other languages such as Italian ~\cite{bianchi2021contrastive}, Korean ~\cite{ko2022large}, Chinese ~\cite{changpinyo2021conceptual, fei2021wenlan, fengshenbang, gu2022wukong, xie2022zero, yang2022chinese} or in a cross-lingual and multilingual setting ~\cite{aggarwal2020towards, carlsson2022cross}.

Training a good language-image representation model often requires a huge amount of text-image pairs and vast computational resources. For instance, CLIP used 400M text-image pairs, and Taiyi ~\cite{fengshenbang}, a recently proposed Chinese model, used 123M text-image pairs. To alleviate this problem, there are multiple works that try to utilize existing pretrained models and only pretrain part of the network ~\cite{portaz2019image, aggarwal2020towards, gu2022wukong, zhai2022lit}. More recently, \newcite{carlsson2022cross} proposed to use Teacher Learning (a.k.a. Knowledge Distillation) on the text encoder of the CLIP model to learn a multilingual text-image representation model. This method only uses machine-translated data from English to a target language, without text-to-image pairs. %We follow this line of work and further improved their method in the following ways.

However, existing works in the cross-lingual or multilingual setting mainly focus on the model's retrieval performance and ignores their generalization ability. The data set to evaluate retrieval performance is often small, e.g., $1,000$ images in test sets for Flickr-30k. The retrieval performance fluctuates acutely with the change in training data distribution. Although current methods achieve good performance in retrieval, these methods often do not perform well on the ImageNet classification tasks. The ability to accurately predict images over $1,000$ classes often indicates better generalization ability of the model. 

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{distillation-framework.pdf}
\caption{\label{fig:framework}The framework of our method.}
\end{figure*}

To address the aforementioned problems, we propose a bilingual model named Alter ego CLIP (\textbf{AltCLIP}) which achieved strong performances on  ImageNet and multimodal retrieval tasks in both English and Chinese. Our AltCLIP learns a strong bilingual language-image representation under a two-stage framework (see Figure \ref{fig:framework} for an overview). In the first stage, we use Teacher Learning to distill the knowledge learned from CLIP. In the second stage, we train the model via Contrastive Learning ~\cite{hadsell2006dimensionality} on a relatively small amount of Chinese and English text-image pairs. We show the effectiveness of our method by experimenting with a wide range of benchmarks in English and Chinese. Further, We set new state-of-the-art results on multiple image classification and retrieval tasks in Chinese. We further extended this method to train a multilingual multimodal model where we call it AltCLIP$_{M9}$. The AltCLIP$_{M9}$ model achieves state-of-the-art zero-shot results on the multilingual text-image retrieval dataset XTD \cite{aggarwal2020zeroshot}.

%Our contributions includes the following:
%\begin{itemize}
%    \item We propose a simple yet effective two-stage method to train a strong bilingual language-image representation model via teacher learning and contrastive learning;
%    \item We achieved state-of-the-art performance on a set of benchmarks in evaluating Chinese Vision-Language models, out-performing models
%    \item We release a benchmark on Chinese Vision-Language tasks and hope to facilitate the evaluation of Chinese Vision-Language models.
%\end{itemize}



==> Bilingual CLIP draft/2_related_work.tex <==
\section{Related Work}
CLIP \cite{radford2021learning} provides a strong English text-image representation. To expand the language of CLIP model,
there are prior studies on learning a bilingual text-image representation ~\cite{ko2022large, bianchi2021contrastive}, and multilingual text-image representation ~\cite{aggarwal2020towards, carlsson2022cross}. In the domain of Chinese text-image pretraining models, prior work such as Taiyi ~\cite{fengshenbang}, CN-CLIP ~\cite{yang2022chinese}, Wukong ~\cite{gu2022wukong}, R2D2 ~\cite{xie2022zero} and BriVL ~\cite{huo2021wenlan, fei2021wenlan}. These methods often need large-scale Chinese text-image pairs and suffer from a significant performance decline in English tasks.
%Most researchers mainly collect large-scale bilingual text-image pairs ($>$100M) to learn the bilingual text encoder from scratch and freeze the parameters of the image encoder.  These works often achieve unsatisfactory performance on zero-shot classifications due to the limited quantity and quality of data beyond English. 

\newcite{carlsson2022cross} proposed a way to utilize Teacher Learning (a.k.a. Knowledge Distillation) \cite{hinton2015distilling} to train a new textual encoder from the original CLIP model with only machine-translated parallel data, without using text-image pairs. Although this method achieves promising cross-lingual retrieval performances with only text data, its zero-shot classification performance in English drops significantly. We follow their work to learn a bilingual model from CLIP with a new text encoder, with the following changes: firstly, we use knowledge distillation on English text pairs in addition to machine-translated text pairs; secondly, we add human-curated translation data for better quality; lastly, we fine-tune the model with text-image pairs to further boost its performance.

%2. Multi-lingual CLIP, Chinese CLIP \\
%In the bilingual setting (Korean and English \cite{ko2022large}, Italian  \cite{bianchi2021contrastive}.

XLM-R \cite{conneau2020unsupervised} is a multilingual language model that achieves strong performances on a wide range of cross-lingual tasks. In our work, we use the XLM-R model as the underlying text encoder and align it with the image encoder trained in CLIP, to achieve competitive performances on cross-lingual and cross-modality tasks. 
%chinese-roberta-wwm \cite{cui2021pre}


==> Bilingual CLIP draft/3_method.tex <==
\section{Methodology} 
We propose a two-stage method to learn a good bilingual and multilingual language-image representation model. In the first stage, we follow the work of \newcite{carlsson2022cross} to use Teacher Learning to learn a multilingual text encoder from the CLIP text encoder. In this step, no image is needed in training and only language parallel data is used. In the second stage, we use text-image pairs to further fine-tune the model from contrastive learning.  Our overall training procedure is summarized in Figure ~\ref{fig:framework}.

%\subsection{Model Architecture}
%As illustrated in Fig.~\ref{fig:framework}, our AltCLIP model has three major components. Firstly, an CLIP text encoder, an CLIP image encoder, and a student text encoder. The CLIP text encoder and CLIP image encoder are adopt from the open available CLIP models. The student text encoder is a language model trained on both English and Chinese data. 

\begin{table*}[htb]
\small
\centering
\begin{tabular}{clccccc} 
\hline
\multirow{2}{*}{Language} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{5}{c}{Dataset}                                         \\ 
\cline{3-7}
                           & \multicolumn{1}{c}{}                         & ImageNet & ImageNet Sketch~ & ImageNet-A & ImageNet-R & ImageNetV2~  \\ 
\hline
\multirow{5}{*}{\rotatebox{90}{English}}   & CLIP                                         & \textbf{75.5}     & \textbf{59.6}             & \textbf{70.6}       & \textbf{87.9}       & \textbf{69.9}         \\
                           & M-CLIP                                       & 52.3     & 44.2             & 59.1       & 81.7       & 47.3         \\
                           %& M-CLIP$_B$                                      & 30       & 22.2             & 21.3       & 48.3       & 26.7         \\
                           & CN-CLIP                                      & 32.5     & 30.7             & 29.8       & 57.0         & 28.6         \\
                           & AltCLIP$_{T}$                                     & 74.7     & 59.2             & 70.4       & 87.9       & 68.8         \\
                           & AltCLIP                                      & 74.5     & 58.7             & 69.5       & 87.2       & 68.2         \\ 
\hline
\multirow{5}{*}{\rotatebox{90}{Chinese}}   & CLIP                                         & 1.9      & 1.7              & 4.7          & 4.4        & 1.8          \\
                           & M-CLIP                                       & 43.0       & 36.3             & 51.3       & 68.3       & 39.5         \\
                           %& M-CLIP$_B$                                      & 23.1     & 17.2             & 16.4       & 38.4       & 20.1         \\
                           & CN-CLIP                                      & 53.6     &47.5           & 42.8       & 78.1       & 47.8         \\
                           & AltCLIP$_{T}$                                     & 58.2     & 46.9             & \textbf{62.7}       & 82.1         & 53.3         \\
                           & AltCLIP                                      & \textbf{59.6}     &\textbf{48.4}             & 61.5       & \textbf{82.5}       &\textbf {54.0}         \\
\hline
\end{tabular}
\caption{Comparison Results of our proposed model and baseline models on image classification benchmarks, i.e. ImageNet and its variants. AltCLIP$_{T}$ and AltCLIP denotes our model after Teacher Learning Stage and after Contrastive Learning Stage, respectively. All image encoders used in these models are Vit-L for fair comparison. The metric reported is zero-shot classification accuracy.}
\label{tab:imagenet}
\end{table*}

\subsection{Teacher Learning Stage}
In this stage, we perform Teacher Learning ~\cite{hinton2015distilling} on text encoders. We use the text encoder from CLIP ~\cite{radford2021learning} as the teacher text encoder, and the XLM-R ~\cite{conneau2020unsupervised} model pretrained on multilingual data as the student encoder. A fully-connected layer is added to transform the output of the XLM-R model into the same output dimension as the teacher encoder. We use parallel text data in both English and Chinese to distill the knowledge of text-image alignment. 

Given parallel text input $(sent_1, sent_2)$, the teacher text encoder generates the learning target from input $sent_1$, which is the embedding of the \ttt{[TOS]} token, denoted by $x^{t}_{tos}$. The student text encoder generates embedding $x^{s}_{cls}$ from input $sent_2$. We minimize Mean Squared Error (MSE) between $x^{t}_{tos}$ and $x^{s}_{cls}$. 
After such training, the student text encoder can keep most of its multilingual capability and obtain text-image alignment capability in both languages. Note that the teacher encoder is only used at training time. At inference time, only the student encoder is used as the text encoder.

To show that our method is extensible at including more languages, we build a multilingual version that supports nine different languages: English(En), Chinese(Zh), Spanish(Es), French(Fr), Russian(Ru), Arabic(Ar), Japanese(Ja), Korean(Ko), and Italian(It). For the multilingual version, we align more languages with English, with the same concept and architecture as in the bilingual version.

%So, we can expand the language of the CLIP model by simply altering the text encoder into the student text encoder. 


\subsection{Contrastive Learning Stage}
This stage of training aims to further improve text-image alignment by contrastive learning on multilingual text-image pairs. As illustrated in Figure \ref{fig:framework}, here we use the image encoder from CLIP which is based on Vision Transformer (ViT) ~\cite{dosovitskiy2020image} as our image encoder, and use the student text encoder learned from the Teacher Learning Stage as our text encoder. 

We use Contrastive Loss ~\cite{hadsell2006dimensionality} between the output projection of the image encoder and text encoder, as done similarly in previous work ~\cite{radford2021learning}. We follow LiT~\cite{zhai2022lit} to freeze the image encoder at training time and only update the parameters in the text encoder. We observe that this stage of training further improves the  model's performance on various evaluation benchmarks, as presented in Section \ref{sec5}.

%\paragraph{Text Encoder}
%We use the original CLIP text encoder as our teacher text encoder. The teacher text encoder generates the learning target, the \ttt{[TOS]} token embedding $x_{tos}$. 

%The student text encoder is a multi-lingual language model that aims to align multi-language inputs to the image encoder. Here, we do not train a multi-lingual CLIP from scratch. Pretraining a non-English CLIP model from scratch is not often applicable~\cite{} due to the imbalance distribution of languages. So, we propose a cross-lingual training schema to learn the cross-lingual text-image alignment ability. After such training, the student model can keep most of its multi-lingual ability and get extra text-image alignment ability. So, we can expand the language of the CLIP model by simply altering the text encoder into the student text encoder. 

%As we know, the quality and quantity of English data are superior to other languages in the world and the English version of CLIP has superior performance than the ones in other languages. 
%Consequently, the text encoder of English CLIP achieves the best alignment ability with the image encoder. To leverage this advantage of English CLIP to expand the input languages of CLIP, we use the text encoder from the CLIP model as the teacher model. 
%By doing so, we can turn a English CLIP into a bi-lingual CLIP with fewer resources. For a given sentence $x$, the CLIP text encoder encode it into a sentence embedding as follow,
%\begin{equation}
%    T_{clip}(x) = x_{tos}\,.
%\end{equation}
%Here, $T_{clip}$ denotes the CLIP text encoder, and $x_{tos}$ represents the embedding of \ttt{[TOS]} token .
%\paragraph{Student Text Encoder}
%For a given sentence $x$, the student text encoder encode it into a sentence embedding as follow,
%\begin{equation}
%    T_{student}(x)=x_{cls}\,.
%\end{equation}
%Here, $T_{student}$ denotes the student text encoder, and $x_{cls}$ represents the embedding of \ttt{[CLS]} token.
%\paragraph{CLIP Image Encoder}
%The image encoder from CLIP model is used as our image encoder. In cross-lingual training schema, the student text encoder will be trained to align multi-language inputs to the CLIP image encoder directly. For a given image $z$, the CLIP image encoder encode it into a image embedding as follow,
%\begin{equation}
%    I_{clip}(z) = z_{cls}\,,
%\end{equation}
%where $I_{clip}$ is the CLIP image encoder, and $z_{cls}$ is the embedding of \ttt{[CLS]} token.

%\subsection{Learning Schema}
%Our training process consists of two stages. The Parallel Teacher Learning (PKD) use the parallel data to distillate the text-image alignment ability from the CLIP model. The Cross-lingual Contrastive Learning (CCL) learn the cross-ligngual text-image alignment in a contrasting manner. 

%\paragraph{Parallel Teacher Learning}
%The Parallel Teacher Learning (PKD) aims to get a multi-lingual text encoder by cross-lingual distillation. The teacher model is the CLIP text encoder which only takes English inputs. The student model  can handle both English and Chinese inputs. Inspired by previous work~\cite{}, we use the student model to learn the cross-lingual text-image alignment by Teacher Learning. We freeze the parameters of teacher model as most study dose. For convelient of training, we use a fully-connected layer to transform the output of student  model into the same output dimension of the teacher model.

%However,  previous methods can not fully take advantage of the text-image alignment of the teacher model and often get unsatisfied performance. To alleviate this problem, we propose the paralleled Teacher Learning. we can get a student model with well text-image alignment and cross-lingual ability.  We formulate the learning procedure as follow, 
%\begin{equation}
%    \ell_{pkd} = \sum_{\{x^{en},x^{cn}\}}\{mse( x^{en}_{cls}, x^{en}_{tos}) + mse(x^{cn}_{cls}, x^{en}_{tos})\}\,.
%\end{equation}
%Here, the $\ell_{pkd}$ is the parallel Teacher Learning loss, $\{x^{en},x^{cn}\}$ is from the parallel data $D_{pkd}$, $x^{en}_{tos}$ is the output of the CLIP text encoder (teacher), $x^{en}_{cls}$ and $x^{cn}_{cls}$ are both the outputs of the student text encoder.
%\paragraph{Cross-lingual contrastive Learning}
%The Cross-lingual Contrastive Learning (CCL) aims to further improve text-image alignment by contrastive learning on multi-lingual text-image pairs. We follow LiT~\cite{zhai2022lit} to freeze the Image tower of CLIP and fine-tuning the parameters in the text encoder. We observe that this further improve the model's performance on zero-shot tasks, as we present in Section \ref{}. The learning procedure is formulated as follow,
%\begin{equation}
%\begin{aligned}
%      \ell_{ccl} = &-\log \frac{\exp{(x\cdot z_+^T/\tau)}} {\sum_{i=1}^{K}\exp{(x \cdot z_i^T/\tau)}}  \\
%    &-\log \frac{\exp{(z \cdot x_+^T/\tau)}} {\sum_{i=1}^{K}\exp{(z \cdot x_i^T/\tau)}} 
%\end{aligned}
%\end{equation}
%Here, $\ell_{ccl}$ is the loss of contrastive learning, $]{x,z]}\in D_{ccl}$, $D_{ccl}$ is the dataset for contrastive learning, $K$ is the batch size. 

==> Bilingual CLIP draft/4_model_training.tex <==
\section{Model Training}
\subsection{Training Datasets} \label{training data}
In this section, we describe the training datasets used in our two-stage model training. 

\paragraph{Teacher Learning Stage}
In this stage, we use parallel text corpus to align the original CLIP text encoder and our new text encoder initialized from XLM-R. Our parallel text corpus includes the following:
\begin{enumerate}

\item Machine translated data of text in Conceptual Captions (CC3M) ~\cite{sharma2018conceptual} and a 28M randomly sampled subset from Laion-400M ~\cite{schuhmann2021laion}. For the multilingual model, we use the same setting but fewer 10M subsets from Laion-400M for each language.
\item Human translated data of text from TSL2019 ~\cite{xu2019nlp}, a total number of 5M English to Chinese translations. For the multilingual model, we extracted the same amount for each language. Parallel data in different languages is extracted from the public database OPUS\cite{tiedemann2012parallel}\footnote{https://opus.nlpl.eu}. This type of parallel data provides more accurate translation.

\end{enumerate}

%In the two stages of training we use different types of data, image-text pairs and parallel-text pairs, respectively. In the Teacher Learning stage we use parallel text to "mock" the teacher's behavior, then in the contrastive learning stage we use image-text pairs to train our text encoder to better fit the image encoder.

%\paragraph{Data For Teacher Learning}
%The parallel corpus used in the Teacher Learning stage consists of machine-translated corpus and human-translated corpus. An intuitive idea is to directly use the captions in the image-text pair as the text corpus, because the data distribution is closer to the data of downstream tasks, such data are representative of CC3M\cite{sharma2018conceptual} and COCO. Another type of data that is far away from downstream tasks is the captions of image-text pairs crawled from the Internet. This type of data is often noisy, and the representative is LAION400M\cite{schuhmann2021laion}. On the other hand, human-translated corpus is also an important parallel corpus. This kind of corpus is characterized by more accurate translation. Our training data combines machine-translated corpora CC3M and Laion28M (a randomly sampled subset of LAION400M) and human-translated corpus TSL2019\cite{xu2019nlp}, totaling 36M Chinese-English parallel text pairs. Captions often require a neural translation model to translate into the target language, and we translate all the English caption into Chinese by using the translation model \cite{TiedemannThottingal:EAMT2020}.

\paragraph{Contrastive Learning Stage}
We use high-quality text-image pair data in this stage. Note that multilingual data are only used in our multilingual version.
%Our text-image  includes the following:
We use 2M bilingual text-image pairs for AltCLIP and 100M multilingual text-image pairs for the multilingual version, from the following:
\begin{enumerate}
\item Chinese text-image dataset from Wudao MM ~\cite{yuan2021wudaocorpora}, filtered by the Laion Aesthetic v2\footnote{https://github.com/christophschuhmann/improved-aesthetic-predictor} model with a threshold score over 5.5.
\item English text-image dataset from LAION 5B ~\cite{schuhmann2022laion}, a randomly sampled subset from the data filtered by the Laion Aesthstic v2 model with a threshold score over 6.

\item Multilingual text-image dataset from LAION Multilingual 2B ~\cite{schuhmann2022laion}, a randomly sampled subset from the data.
\end{enumerate}
%The total number of text-image pairs we used is 11M. 
%We use a subset of 2M text-image pairs from the above.
%The image-text pair data used in the contrastive learning phase is the parallel pair of Chinese captions and images. At this stage we tend to use higher-quality image-text pair data, and we use the Laion aesthetic model to pick out high-quality image-text pairs. Specifically, we select image-text pairs with an aesthetic score higher than 5.5 points from the Chinese open source multimodal dataset Wudao\cite{yuan2021wudaocorpora} and image-text pairs with an aesthetic score higher than 6 points from Laion Aesthetics v2. A total of 2M image-text pairs are used for comparative learning.

\begin{table*}[hbt]
\centering
\small
\begin{tabular}{ccccccccc}\hline
\multirow{2}{*}{Dataset}   & \multirow{2}{*}{Method} & \multicolumn{3}{l}{Text-to-Image Retrival} & \multicolumn{3}{l}{Image-to-Text Retrival} & \multirow{2}{*}{MR} \\\cline{3-8}
                           &                         & R@1          & R@5          & R@10         & R@1          & R@5          & R@10         &                     \\\hline
\multirow{7}{*}{\rotatebox{90}{Flickr30k$_{EN}$}} & CLIP         &    65.0          &     87.1         &      92.2        &    85.1          &      97.3        &    \textbf{99.2}          &  87.6                   \\
& Taiyi &25.3	&48.2	&59.2	&39.3	&68.1	&79.6	&53.3 \\ 
& Wukong &-	&-	&-	&-	&-	&-	&- \\
& R2D2 &-	&-	&-	&-	&-	&-	&-\\
& CN-CLIP & 49.5	&76.9	&83.8	&66.5	&91.2 	&96.0	&77.3 \\
& AltCLIP$_{T}$ &66.3	&87.8	&\textbf{92.7}	&85.9	&97.7	&99.1	&88.3 \\
& AltCLIP &\textbf{72.5}	&\textbf{91.6}	&\textbf{95.4}	&\textbf{86.0}	&\textbf{98.0}	&99.1 &	\textbf{90.4} 
               \\\hline
\multirow{7}{*}{\rotatebox{90}{Flickr30k$_{CN}$}} & CLIP         &       0      &      2.4        &     4.0         &     2.3         &   8.1           &     12.6        &    5.0                 \\
& Taiyi &53.7	&79.8	&86.6	&63.8	&90.5	&95.9	&78.4 \\
& Wukong$^{\dag}$ &51.7	&78.9	&86.3	&76.1	&94.8	&97.5	&80.9 \\
& R2D2$^{\dag}$ &60.9	&86.8	&92.7	&77.6	&96.7	&\textbf{98.9}	&85.6 \\
& CN-CLIP &68	&89.7	&94.4	&80.2	&96.6	&98.2	&87.9 \\
& AltCLIP$_{T}$&63.7	&86.3	&92.1	&84.7	&97.4	&98.7	&87.2 \\
& AltCLIP &\textbf{69.8}	&\textbf{89.9}	&\textbf{94.7}	&\textbf{84.8}	&\textbf{97.4}	&98.8	&\textbf{89.2}   
\\\hline

\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{EN}$}} & CLIP
               &36.5 &61.1  &71.1 &56.4 &79.5  &86.5  &65.2\\
&Taiyi &11.7 &27.8  &37.4 &19.8 &42.1  &54.3  &32.2 \\ 
&Wukong &-	&-	&-	&-	&-	&-	&- \\
&R2D2 &-	&-	&-	&-	&-	&-	&-\\
  
&CN-CLIP  &26.1 &50.0  &61.3 &40.9 &65.8  &76.3  &53.4\\
&AltCLIP$_{T}$&37.5 &62.1  &72.1 &57.2 &80.5  &87.5  &66.1  \\
&AltCLIP&\textbf{42.9} &\textbf{68.0}  &\textbf{77.4} &\textbf{58.6} &\textbf{80.6}  &\textbf{87.8}  &\textbf{69.2} 

               \\\hline
\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{CN}(1K)$}} & CLIP  &0.6 &4.1  &7.1 &1.8 &6.7  &11.9  &5.4 \\
&Taiyi&52.0 &80.2  &89.6 &46.6 &76.3  &88.6  &72.2  \\
&Wukong$^{\dag}$ &55.2& 81.0 &90.6 &53.4 &80.2 &90.1 &75.1 \\
&R2D2$^{\dag}$ &63.3 &\textbf{89.3} &\textbf{95.7} &56.4 &85.0 &93.1 &80.5 \\
&CN-CLIP &63.7 &88.7  &94.4 &61.0 &84.7  &93.6  &81.0 \\

&AltCLIP$_{T}$&55.7 &82.9  &91.2 &60.7 &86.3  &93.4  &78.4  \\
&AltCLIP&\textbf{63.9} &87.2  &93.9 &\textbf{62.8} &\textbf{88.8}  &\textbf{95.5}  &\textbf{82.0} 

\\\hline
\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{CN}(5K)$}} & CLIP  &0.8 &3.9  &5.8 &3.5 &8.9  &14.4  &6.2    \\
& Taiyi &46.1 &74.9  &85.1 &58.1 &83.9  &91.7  &73.3   \\
&Wukong &-	&-	&-	&-	&-	&-	&- \\
&R2D2&-	&-	&-	&-	&-	&-	&- \\
&CN-CLIP &58.6 &85.3  &92.7 &72.1 &90.9  &94.7  &82.4 \\
&AltCLIP$_{T}$ &54.9 &81.8  &90.5 &76.3 &93.9  &\textbf{97.6}  &82.5  \\
&AltCLIP&\textbf{61.3} &\textbf{86.0}  &\textbf{93.2} &\textbf{77.8} &\textbf{94.4}  &97.5  &\textbf{85.0} 
\\\hline
\end{tabular}
\caption{Experimental results on retrieval tasks, namely English and Chinese version of Flickr30k and MSCOCO. All image encoders used in these models are ViT-L for fair comparison. AltCLIP$_{T}$ denotes our model after Teacher Learning stage while AltCLIP denotes our model after contrastive learning stage.$^{\dag}$ represents we report original results from papers.}
\label{tab:retrieval}
\end{table*}


\subsection{Implementation details}
We initialize our text encoder from XLM-R$_{Large}$. We use the text encoder from CLIP$_{ViT-L14}$ as the teacher text encoder, and the image encoder of the same CLIP model as our image encoder. 
%Starting from the pre-trained model XLM-Roberta-Large ~\cite{conneau2020unsupervised}. See the table\ref{table:model} for specific model parameter details. 
%We freeze parameters of CLIP (including text projection layer and image projection layer). 
For specific hyper-parameter settings in our two-stage training, please refer to the table \ref{tab:hyper} in Appendix.
%As described in section \ref{training data}, we trained both models using the same data. Additionally, except for the language encoder, we froze the pre-trained parameters of CLIP (including text projection layer and image projection layer). For specific hyper-parameter settings, please refer to the table \ref{table:hpparameters}


\begin{figure*}[htp]
    \centering
    \includegraphics[scale=0.75]{figures/6_clipbcm}
    \caption{Comparison Results of our proposed model and OpenAI's CLIP. AltCLIP$_{T}$ denotes for our model after Teacher Learning Stage while AltCLIP denotes for our model after Contrastive Learning Stage. AltCLIP$_{M9}$ denotes for our model extending to 9 different languages. All image encoders are CLIP$_{ViT-L14}$. }
    \label{fig:clipbcm}
\end{figure*}


==> Bilingual CLIP draft/5_experiments.tex <==
\section{Experiments}
\label{sec5}
We present our experimental results in this section. In Section \ref{sec5-1}, we introduce the datasets and metrics used in the evaluation. We comprehensively validate our model through zero-shot benchmarks in both English and Chinese in Section \ref{sec5-2}.
%We consider both bilingual and monolingual scenarios, to comprehensively validate the language capabilities, through zero-shot performances. We then present the general performances on the selected benchmarks to compare AltCLIP and the state-of-the-art image-text models. 
In Section \ref{sec5-3}, we conduct an ablation study on the effects of various design choices in Teacher Learning and Contrastive Learning. 
Finally, in Section \ref{sec5-4}, we use an AltCLIP-guided diffusion model to generate images from both Chinese and English prompts, and show that our model is capable to align text in different languages.
%In addition, examples of generated images from bilingual text prompts through AltCLIP-guided diffusion model are shown to ``visualize" the language capabilities.

%As mentioned above, we perform evaluations on both bilingual and monolingual benchmarks. 

%Bilingual benchmarks require image collections with associated parallel bilingual texts.
%\ledell{Here we should say ImageNet is an important benchmark for evaluating Vision pretraining model, instead of 'we have the translation'}
\subsection{Evaluation Datasets and Metrics} 
\label{sec5-1}
In this section, we describe the datasets and metrics we used in our experiments. We use ImageNet ~\cite{deng2009imagenet} and its four out-of-distribution test variants, i.e. ImageNet Sketch~\cite{wang2019learning}, ImageNet-A~\cite{hendrycks2021natural}, ImageNet-R~\cite{hendrycks2021many}, ImageNetV2~\cite{recht2019imagenet}, to evaluate zero-shot image classification performances in English and Chinese. \footnote{We use the Chinese translation of classnames from \url{https://github.com/ningbonb/imagenet_classes_chinese}}
%ImageNet is widely-applied to assess consistent performances on natural distributions for vision pretraining models.
During evaluation, we adapt the templates of manual prompts from CLIP for English and corresponding machine translation templates for Chinese. For cross-modal retrieval, we select Flickr30k~\cite{young2014image}, MSCOCO~\cite{lin2014microsoft}, as well as their corresponding Chinese datasets, Flickr30k$_\text{CN}$~\cite{lan2017fluency}, MSCOCO$_\text{CN}$~ \footnote{two versions, texts in 1k version are manual written captions while in 5k version are manual translated captions}~\cite{li2019coco}, to evaluate zero-shot image-to-text retrieval and text-to-image retrieval performances. 

We further validate our model on a wide range of tasks to compare the performance with the original CLIP model. We collect the datasets introduced in CLIP and the Open CLIP benchmark \footnote{\url{https://github.com/LAION-AI/CLIP_benchmark}}, including Birdsnap~\cite{berg2014birdsnap}, Caltech-101~\cite{fei2006one}, Stanford Cars~\cite{Krause2013}, CIFAR-10~\cite{krizhevsky2009learning}, CIFAR-100~\cite{krizhevsky2009learning}, Country211~\cite{radford2021learning}, DTD~\cite{cimpoi2014describing}, EuroSAT~\cite{helber2019eurosat}, Facial Emotion Recognition 2013~\cite{goodfellow2013challenges}, FGVC Aircraft~\cite{blaschko2012towards}, Oxford Flowers 102~\cite{nilsback2008automated}, Food-101~\cite{bossard14}, GTSRB~\cite{stallkamp2011german}, Kinetics400~\cite{kay2017kinetics}, Kinetics600~\cite{carreira2018short}, MNIST~\cite{cirecsan2011high}, PatchCamelyon~\cite{veeling2018rotation}, ObjectNet~\cite{barbu2019objectnet}, Oxford-IIIT Pets~\cite{parkhi2012cats}, Rendered SST2~\cite{radford2021learning}, RESISC45~\cite{cheng2017remote}, STL-10~\cite{coates2011analysis}, SUN397~\cite{Xiao2010}, UCF101~\cite{soomro2012ucf101}, Pascal VOC 2007 Classification~\cite{pascal-voc-2007}, Pascal VOC 2007 Multilabel Classification~\cite{pascal-voc-2007}. 
%Additionally, more monolingual benchmarks are introduced in order to compare the performance on wider distributions and tasks with CLIP. 
%These datasets are collected from the well-studied evaluation introduced in CLIP ~\cite{radford2021learning} and the Open CLIP benchmark\footnote{\url{https://github.com/LAION-AI/CLIP_benchmark}}, an open-source project to evaluate Language-Image pretraining models, including Birdsnap, Caltech-101, Stanford Cars, CIFAR-10, CIFAR-100, Country211, DTD, EuroSAT, Facial Emotion Recognition 2013, FGVC Aircraft, Oxford Flowers 102, Food-101, GTSRB, Kinetics400, Kinetics600, MNIST, PatchCamelyon, Oxford-IIIT Pets, Rendered SST2, RESISC45, STL-10, SUN397, UCF101, Pascal VOC 2007 Classification, Pascal VOC 2007 Multilabel Classification. 
Finally, we evaluate our multilingual model AltCLIP$_{M9}$ on the \textbf{XTD} ~\cite{aggarwal2020zeroshot} dataset. XTD selected 1K images from MS COCO, and translated the corresponding English Captions into 11 languages (English(en), German(de), French(fr), Chinese(zh), Japanese(ja), Italian(it), Spanish(es), Russian(ru), Polish(pl), Turkish(tr), Korean(ko)).
The evaluation metrics for image classification benchmarks are respectively accuracy (default), mean per class (the average of recall obtained on each class, for imbalanced datasets, i.e. FGVC Aircraft, Oxford-IIIT Pets, Caltech-101, Oxford Flowers 102), 11-point mAP (mean average of 11-pt interpolated precision for each class, for VOC 2007), mean(top1, top5) (the mean of acc@1 and acc@5, for Kinetics400 and Kinetics600), while for cross-modal retrieval benchmarks, are Recall@K where $K\in\{1,5,10\}$, and Mean Recall(MR, i.e., the average of
Recall@K) for both image-to-text retrieval and text-to-image retrieval tasks, which are same with the setups in CLIP ~\cite{radford2021learning}.



\begin{table*}[t]
\centering
\small
\begin{tabular}{ccccccccc} 
\hline
\diagbox{Method}{Language} & En            & Es            & Fr            & Zh            & It            & Ko            & Ru            & Jp             \\ 
\hline
CLIP$_{ViT-B32}$                       & 90.3          & -             & -             & -             & -             & -             & -             & -              \\
CLIP$_{ViT-L14}$                       & 91.8          & -             & -             & -             & -             & -             & -             & -              \\
CLIP$_{ViT-B16+}$$\dag$                       & 94.3          & -             & -             & -             & -             & -             & -             & -              \\
mUSE PATR                      &83.6  &75.6 &76.9 &76.1 &73.4 &64.3 &73.6  &69.4            \\
mUSE m3             &85.3  &78.9 &78.9 &76.7 &73.6 &67.8 &76.1  &70.7         \\
M-CLIP$_{ViT-B32}$                     &91.8		&89.1	&89.4	&89.3	&89.8		&82.1	&86.1		&81.0           \\
M-CLIP$_{ViT-L14}$                     & 92.4          & 91            & 90            & 89.7          & 91.1          & 85.2          & 85.8          & 81.9           \\
M-CLIP$_{ViT-B16+}$$\dag$      &95   &93.6	&\textbf{93.1}	&94	&93.1		&89	&90	&84.2      \\
%AltCLIP$^T_{M9}$                & 94.7          & 91.2          & 91.3          & 93.7          & 92.9          & 92.7          & 89.9          & 89.8           \\
AltCLIP$_{M9}$                    & \textbf{95.4} & \textbf{94.1} & 92.9 & \textbf{95.1} & \textbf{94.2} & \textbf{94.4} & \textbf{91.8} & \textbf{91.7}  \\
\hline
\end{tabular}
\caption{Comparison results on the multilingual cross-modal Retrieve dataset XTD.  Following M-CLIP, we report recall@10 on Image to Text. \dag  represents using image encoder released by OpenCLIP project ~\cite{ilharco_gabriel_2021_5143773}. 
%We report all result from official report. 
\label{tab:xtd}}
\end{table*}
% \begin{table*}[tb]
% \small
% \centering
% \begin{tabular}{ccccccc}\hline
% EN-EN & EN-CN & Both & Flickr30k$_{EN}$ & Flickr30k$_{CN}$ & ImageNet$_{EN}$ & ImageNet$_{CN}$ \\\hline
% %CN-Our-xmlr  & Laion28m          &                   &                            & 87.01        & 5.5          & 70.3        & 2           \\
%  \Checkmark             &                   &                              & 86.59        & 53.86        & 53.76       & 12.84       \\
%                      & \Checkmark             &                              & 61.89        & 85.37        & 15.47       & 42.47       \\
% % \Checkmark             & \Checkmark              &                              & 79.82        & 85.60         & 32.77       & 42.20        \\
%                      &                     & \Checkmark                   & 86.82        & 85.84        & 51.61       & 41.66       \\\hline
% %CN-Ours-xmlr &                   &                   & Laion28M                   & 87.76        & 86.05        & 73.85       & 46.21      \\\hline
% \end{tabular}
% \caption{Ablation Experiments on parallel text used in Teacher Learning. En-En indicates the use of English-English text pairs; En-Cn indicates the use of English-Chinese parallel text. \label{tab:pkd}}
% \end{table*}
% \usepackage{booktabs}


\begin{table*}[tb]
\centering
\small
\begin{tabular}{cccc|cccc} 
\toprule
EN-EN & EN-CN$_{MT}$ & EN-CN$_{HT}$ & CL             & \multicolumn{1}{l}{Flickr30K$_{EN}$} & \multicolumn{1}{l}{Flickr30K$_{CN}$} & \multicolumn{1}{l}{ImageNet$_{EN}$} & \multicolumn{1}{l}{ImageNet$_{CN}$}  \\ 
\midrule
\Checkmark                &\Checkmark&\Checkmark&\Checkmark& \textbf{90.4}                                 & \textbf{89.2}                                   & 74.5                                & \textbf{59.6}                           \\

\Checkmark             &\Checkmark&\Checkmark&& 88.3                                 & 87.2                                   & \textbf{74.7}                                & 58.2                                 \\

\Checkmark &\Checkmark&&& 86.8                                & 85.8                                  & 51.6                               & 41.7                                \\

\Checkmark  &&&& 86.6                                & 53.9                                  & 53.8                               & 12.8                                \\

   &\Checkmark&&& 61.9                               & 85.4                                  & 15.5                               & 42.5                                \\
% \quad -w/ EN\&CN & 86.8                                & 85.8                                  & 51.6                               & 41.7                                \\
\bottomrule
\end{tabular}
\caption{Ablation Experiments. CL indicates the use of Contrastive Learning stage, while EN-EN, \text{EN-CN}$_{MT}$, \text{EN-CN}$_{HT}$ refers to parallel data used in Teacher Learning stage. Specifically, EN-EN indicates the use of English-English text pairs; EN-CN indicates the use of English-Chinese parallel text, including \text{EN-CN}$_{MT}$ represents machine translated pairs while \text{EN-CN}$_{HT}$ stands for human-translated data, i.e TSL2019. All compared models are pre-trained for 10 epochs. $\label{tab:pkd}$}
\end{table*}

% \begin{table*}[tb]
% \centering
% \begin{tabular}{l|cccc} 
% \toprule
% Methods             & \multicolumn{1}{l}{Flickr30K$_{EN}$} & \multicolumn{1}{l}{Flickr30K$_{CN}$} & \multicolumn{1}{l}{ImageNet$_{EN}$} & \multicolumn{1}{l}{ImageNet$_{CN}$}  \\ 
% \midrule
% Ours                & \textbf{90.4}                                 & \textbf{89.2}                                   & 74.5                                & \textbf{59.6}                           \\
% -w/o CL             & 88.3                                 & 87.2                                   & \textbf{74.7}                                & 58.2                                 \\
% -w/o CL\&Parallel Data & 86.8                                & 85.8                                  & 51.6                               & 41.7                                \\
% \quad -w/ EN-EN  & 86.6                                & 53.9                                  & 53.8                               & 12.8                                \\
% \quad -w/ EN-CN   & 61.9                               & 85.4                                  & 15.5                               & 42.5                                \\
% % \quad -w/ EN\&CN & 86.8                                & 85.8                                  & 51.6                               & 41.7                                \\
% \bottomrule
% \end{tabular}
% \caption{Ablation Experiments. CL indicates the use of Contrastive Learning and Parallel Data refers to human-translated data, i.e TSL2019. EN-EN indicates the use of English-English text pairs; EN-CN indicates the use of English-Chinese parallel text; EN\&CN indicates the use of English-Chinese parallel text and English-English parallel text. All compared models are pre-trained for 10 epochs. $\label{tab:pkd}$}
% \end{table*}


\subsection{Zero-shot performance}
\label{sec5-2}
%of AltCLIP with CLIP and CN-CLIP, which are respectively the previous sota English and Chinese CLIP-like model as far as we know.
%As illustrated in Table~\ref{tab:imagenet}, AltCLIP, regardless of after Teacher Learning process or contrastive learning process, achieve sota or nearly sota accuracy on both English and Chinese image classification benchmarks. On the contrary, the performances of  CLIP and CN-CLIP on the same image collections collapse, when switching the text to another language. Specifically, compared with CLIP, the average accuracy of AltCLIP on English datasets is only slightly lower, while on Chinese datasets, AltCLIP outperforms CLIP by a large margin, over 50.0 absolute average accuracy. Moreover, compared to CN-CLIP, on both languages, AltCLIP achieves better accuracy on almost all datasets, except the Chinese ImageNet Sketch Dataset. The statistics show both the extended Chinese language capabilities and consistent English language capabilities.
\paragraph{Image Classification}
We first present evaluation results of zero-shot image classification on the ImageNet dataset and its four out-of-distribution variants. For baselines, we compare our model with CLIP ~\cite{radford2021learning}, CN-CLIP ~\cite{yang2022chinese}, and multilingual CLIP (M-CLIP) ~\cite{carlsson2022cross}.
As illustrated in Table~\ref{tab:imagenet}, AltCLIP achieves results that are very close to CLIP in English and sets new state-of-the-art results on Chinese ImageNet, ImageNet-A, ImageNet-R, and ImageNet V2. These results demonstrate the effectiveness of our method: compared to other Chinese baseline models where hundreds of millions of text-image pairs are used in pretraining, we only use 36M parallel text data and 2M text-image pairs in training.

\paragraph{Cross-modal Retrieval}
For cross-modal retrieval, we compare our model with CLIP in English and R2D2 ~\cite{xie2022zero}, Wukong ~\cite{gu2022wukong}, Taiyi ~\cite{fengshenbang} and CN-CLIP ~\cite{yang2022chinese} in Chinese. The results are shown in Table~\ref{tab:retrieval}. AltCLIP outperforms all baseline models on most datasets and tasks. We notice that AltCLIP outperforms CLIP on both text-to-image and image-to-text retrieval. This could be due to the following reasons: 1). We used a small subset (less than 1M) of LAION 5B at the Contrastive Learning stage, which is in a different distribution of the pretraining data used in CLIP; 2). Our language encoder initialized from XLM-R provides better language understanding ability. We left it as a future investigation to properly analyze the factors.

%An interesting phenomenon is that on English datasets, AltCLIP outperforms CLIP on both text-to-image retrieval and image-to-text retrieval. This might indicate that the proposed approach, extends the language capabilities, by not only increasing the comprehension of target language, but also improving the matching abilities of image and source language.
\paragraph{Multilingual Cross-modal Retrieval}
%In order to evaluate the scalability of our method, we expanded the language to 8 languages, namely English(En), Chinese(Zh), Spanish(Es), French(Fr), Russian(Ru), Japanese(Ja), Korean(Ko), and Italian(It).
% Different from the above bilingual experiment, we translate LAION10M(subset of LAION400M) and CC3M and add 5M parallel corpus for each language. 
For baseline, we compare our model with CLIP, M-CLIP ~\cite{carlsson2022cross} and mUSE ~\cite{yang-etal-2020-multilingual}. The results of the comparison on XTD ~\cite{aggarwal2020zeroshot} are shown in Table \ref{tab:xtd}, where AltCLIP$_{M9}$ achieves state-of-the-art results in 7 languages. Notably, joint multilingual training maintains state-of-the-art capabilities in English and achieves better results than the original CLIP model on this dataset. We may achieve better results for two reasons: 1. We equally translate a fixed set of English captions for each language, which allows each language to share a more comprehensive distribution. 2. We introduce more parallel data of human translation, and experiments show that this part of the data is helpful for establishing a robust multilingual representation.
%demonstrating the linguistic scalability of our method.

\paragraph{Full CLIP benchmark}
We present the evaluation results of a wider range of tasks in English in Figure \ref{fig:clipbcm}. We compare the effectiveness of the Teacher Learning Stage and Contrastive Learning Stage, and the bilingual AltCLIP and multilingual AltCLIP$_{M9}$. We observe that at the Teacher Learning Stage, the model already learns a good representation of text-image representation, as it gets a close performance of the original CLIP model on a broad range of zero-shot benchmarks. The Contrastive Learning stage further improves our model’s performance, especially on retrieval tasks like Flickr30k and MSCOCO. Further, the multilingual AltCLIP$_{M9}$ achieves close performances with bilingual AltCLIP, indicating that our method is effective at extending the number of languages supported.

\subsection{Ablation study}
\label{sec5-3}
In this section, we present results from ablation studies. We show the significance of including various parallel data in Teacher Learning stage in Table \ref{tab:pkd}. As illustrated in the 3rd and 5th line, without English-to-English parallel data, the accuracy on English ImageNet drastically drops to 15.47 from 53.8. Similarly, excluding machine-translated English-to-Chinese data, has a great impact on the performances on Chinese benchmarks, i.e. Imagenet$_{CN}$ and Flickr30K$_{CN}$, due to influenced Chinese text-image representation. Moreover, empirical experiments show that introducing human translated parallel data leads to a great improvement on Imagenet$_{CN}$ which may be related to the distribution of the data set. This indicates that the diversity of training data used for teacher learning, can benefit the language model to gain more knowledge about entities or concepts.

%To evaluate our proposed two-stage training methods, we design several setups for the ablation study. Firstly, we evaluate the effects of our proposed distillation using XLM-R-base as student model. Secondly, we evaluate the effects of cross-lingual contrastive learning with the XLM-R-large model.
%\paragraph{Effects of parallel Teacher Learning}
%To effects of parallel Teacher Learning, we conduct a set of experiments under different parallel data settings.  As show in Tab.~\ref{tab:pkd}, the experimental results demonstrates that our proposed method can get a student model with well text-image alignment and cross-lingual abilities. 
%\paragraph{Effects of cross-lingual contrastive learning}
%To evaluate our proposed cross-lingual contrastive learning, we conduct a group of experiments with different contrastive learning settings. As show in Tab.~\ref{tab:ccl}, the cross-lingual contrastive learning help the model achieve significant higher performance on retrival tasks, e.g. Flickr30k and MSCOCO.

\subsection{Examples of text-to-image generation}
\label{sec5-4}
To demonstrate the effects of text alignment in our model, we use the text encoder of AltCLIP and AltCLIP$_{M9}$ to further finetune a text-to-image generation model from Stable Diffusion ~\cite{rombach2022high}.
We use stable-diffusion v1-4\footnote{https://huggingface.co/CompVis/stable-diffusion-v-1-4-original} as initialization, and we use AltCLIP or AltCLIP$_{M9}$ as the language encoder. We freeze all the parameters in the diffusion model except for the key and value projection layers of the cross-attention block during finetuning. The dataset we used to finetune is the same one used for Contrastive Learning as described in Section \ref{training data}. We call our image generation models AltDiffusion and AltDiffusion$_{M9}$. 

%We use the pre-trained bilingual language model as our text encoder and fine-tune it using the WuDao dataset (6M) with an aesthetic score above 5.5 and the Laion data (5M) with an aesthetic score above 5.5.

As shown in Fig.~\ref{fig:demo}, AltDiffusion generates high-quality images close to Stable Diffusion on both English and Chinese prompts. Further, we notice that our model generates very similar images given translated English and Chinese prompts. For the multilingual version, we observed a very interesting phenomenon: when given a prompt that’s translated into different languages, the generated images reflect cultural differences to some extent. See Tab. ~\ref{tab:m9} for some examples. We left it as a future effort to explore and analyze carefully on how culture inherited in different languages can affect image generation.

%As illustrated in Tab.~\ref{tab:m9}, our model generates images reflecting the culture in different languages. For example, Russian girls have very Russian-style head wears.

\begin{figure}
    \centering
    \subfigure[Stable Diffusion]{
    \includegraphics[width=0.45\textwidth]{figures/1_sd.jpg}
    }
    \subfigure[AltDiffusion EN]{
    \includegraphics[width=0.45\textwidth]{figures/2_our.jpg}
    }
    \subfigure[AltDiffusion CN]{
    \includegraphics[width=0.45\textwidth]{figures/3_our_zh.jpg}
    }
    %\subfigure[An Open source bi-lingual Stable Diffusion EN]{
    %\includegraphics[width=0.45\textwidth]{figures/4_taiyi.jpg}
    %}
    %\subfigure[An Open source bi-lingual Stable Diffusion CN]{
    %\includegraphics[width=0.45\textwidth]{figures/5_taiyi_zh.jpg}
    %}
    \caption{Examples of text-to-image generation. Text prompt: \textit{"a pretty female druid surrounded by forest animals, digital painting, photorealistic, in the style of greg rutkowski, highly detailed, realistic.",\begin{CJK}{UTF8}{gbsn} "一个由森林动物环绕的漂亮的女德鲁伊,数字绘画,摄影现实,格雷格·鲁特科夫斯基风格,高度详细,现实"\end{CJK}} \label{fig:demo}}
    \label{fig:my_label}
\end{figure}

\begin{table*}[]
    \centering
    \begin{tabular}{b{0.25\linewidth}|p{0.65\linewidth}}\hline
        Prompts & Generated Image \\\hline
        \includegraphics[width=0.95\linewidth]{figures/m9/ent.png}  & \includegraphics[width=1\linewidth]{figures/m9/en.png}\\
      \includegraphics[width=0.95\linewidth]{figures/m9/zht.png}  & \includegraphics[width=1\linewidth]{figures/m9/zh.png}\\
      \includegraphics[width=0.95\linewidth]{figures/m9/frt.png}  & \includegraphics[width=1\linewidth]{figures/m9/fr.png}\\
      \includegraphics[width=0.95\linewidth]{figures/m9/spt.png}   & \includegraphics[width=1\linewidth]{figures/m9/sp.png}\\
       \includegraphics[width=0.95\linewidth]{figures/m9/rut.png}  & \includegraphics[width=1\linewidth]{figures/m9/ru.png}\\
        \includegraphics[width=0.95\linewidth]{figures/m9/art.png}  & \includegraphics[width=1\linewidth]{figures/m9/ar.png}\\
         \includegraphics[width=0.95\linewidth]{figures/m9/jat.png}   & \includegraphics[width=1\linewidth]{figures/m9/ja.png}\\
          \includegraphics[width=0.95\linewidth]{figures/m9/kot.png}   & \includegraphics[width=1\linewidth]{figures/m9/ko.png}\\
           \includegraphics[width=0.95\linewidth]{figures/m9/itt.png}   & \includegraphics[width=1\linewidth]{figures/m9/it.png}\\\hline
    \end{tabular}
    \caption{The images generated by AltDiffusion$_{M9}$ with the same prompt translated to nine languages and a fixed seed.}
    \label{tab:m9}
\end{table*}
%\begin{figure}
%\centering
%\subfigure[Stable Diffusion] {
%\includegraphics[width=0.45\textwidth]{figures/sd_better.jpg}
%}
%\subfigure[AltDiffusion] {
%\includegraphics[width=0.45\textwidth]{figures/2_our_better.jpg}
%}
%\caption{Example of bilingual text-to-image generation. Text prompt: 
%\textit{"穿着唐朝服装, 唐朝, lofi Uraraka from My Hero Academia portrait, Pixar style, by Tristan Eaton Stanley Artgerm and Tom Bagshaw."}. The Chinese part in the prompt is translated to \textit{"Wearing Tang Dynasty clothing, Tang Dynasty"} for Stable Diffusion.
%}
%\label{fig:better_than_sd}
%\end{figure}


% \begin{table*}[bhtp]
% \centering
% \begin{tabular}{cc|ccccccc}\hline
% %Language & Dataset          & CLIP$_{\text{ViT-L}}$   &CN-CLIP$_\text{ViT-L}$  & AltCLIP$_\text{ViT-L}_{K}$ & AltCLIP^*$_\text{ViT-L}$ \\\hline
%  & Dataset          & CLIP & M-CLIP & M-CLIP$_{B}$ &CN-CLIP  &Wukong & AltCLIP$_{T}$ & AltCLIP  \\\hline
% \multirow{5}{*}{\rotatebox{90}{English}} &ImageNet    & \textbf{75.5} &52.3  &30  &32.5  &-  & 74.7           & 74.5      \\
% &ImageNet Sketch       & \textbf{59.6}  &44.2 &22.2   &30.7  &- & 59.2           & 58.7      \\
% &ImageNet-A             & \textbf{70.6} &59.1 &21.3 &29.8   &-  & 70.4           & 69.5      \\
% &ImageNet-R             & \textbf{87.9} &81.7  &48.3 &57.0  &-  & \textbf{87.9 }          & 87.2      \\
% &ImageNetV2             & \textbf{69.9} &47.3 &26.7  &28.6  &-  & 68.8           & 68.1      \\ \hline
% \multirow{5}{*}{\rotatebox{90}{Chinese}} & ImageNet   &  1.9  &43. &23.1 & 53.6    &58.2  &   58.2         &  \textbf{59.6}     \\
% & ImageNet Sketch                       &  1.9 &36.8 &17.2  &\textbf{47.3} & - &     44.5       &  46.5     \\
% &ImageNet-A                             & 6.0 &51.7 &16.4 & 43.1   &-  &     56.8       &   \textbf{58.5}    \\
% &ImageNet-R                              & 5.3 &68.7 &38.4 & 77.6  &-   &     78.0       &  \textbf{79.9 }    \\
% & ImageNetV2                             &  1.8 &40.1 &20.1 & 48.3 &-    &     48.1      &   \textbf{50.9}    \\ \hline
% \end{tabular}
% \caption{Comparison Results of our proposed model and sota CLIP models on image classification benchmarks, i.e. ImageNet and its variants. AltCLIP$_{T}$ and AltCLIP are the same to Figure 2. All image encoders used in these models are Vit-L for fair comparison. The metric reported is zero-shot classification accuracy.}
% \label{tab:imagenet}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}






==> Bilingual CLIP draft/6_conclusion.tex <==
\section{Conclusion}
In this work, we presented a conceptually simple and effective two-stage training schema to learn bilingual and multilingual multimodal representation models, via teacher learning and contrastive learning. We show the effectiveness of our method by conducting extensive experiments on a wide range of tasks in English and Chinese. In Chinese, our method sets new state-of-the-art results on multiple zero-shot image classification and retrieval tasks while being highly effective: we only use tens of millions of text data and two million text-image pairs during training, whereas most prior work requires training on hundreds of millions of text-image pairs. Future work includes exploring altering the image encoder to combine vision signals learned from different data distributions and possibly eliminating the need for machine-translated data to build a multilingual multimodal pretraining model.

%Learning a good representation in a joint space for vision and language has been a long pursuit in the research of Artificial Intelligence (AI). Recently, the milestone work of CLIP \cite{clip} from OpenAI demonstrated impressive zero-shot performances across a number of tasks such as Image classification on ImageNet, Image-to-Text and Text-to-Image retrieval on Flicker-30K, MSCOCO, . There has been pursuit of contrastive language-image model in other languages such as Italian, Korean, Chinese or in a cross-lingual/multi-lingual setting \cite{}.

%Training a language-image representation usually require a large number of text-image pairs (for instance, CLIP used 400M text-image pairs, and Taiyi, a Chinese CLIP model, used 123M text-image pairs), and a huge number of computing resources where most research groups don’t have access to.  \cite{} Proposed a novel technique to Teacher Learning (a.k.a. Knowledge Distillation) on the textual encoder of the CLIP model, which only require machine-translated data from English to target language, without text-to-image pairs. We follow this line of work and further improved their method in the following ways.

%We proposed a simple, scalable, and effective two stage approach for learning a good Chinese CLIP model while keeping the same capability.
%Notably, we achieved on-par performance on image retrieval tasks for both English and Chinese. However, the results on Imagnet differs a lot: while CLIP achieves xxx on ImageNet~\cite{deng2009imagenet} classification, our model drops at an accuracy of 59.xx\% on Imagnet-cn. We suspect this is due to xxx. We left it as future direction to close this gap on Imagnet between English and Chinese.



==> Bilingual CLIP draft/7_acknowledgement.tex <==
\section*{Acknowledgements}
We’d like to thank Yizhou Zheng for helpful suggestions on fine-tuning stable diffusion models. We’d like to thank Luke Zettlemoyer for valuable suggestions and advices. We also thank Chenghua Zhou, Quan Sun and Yue Cao for helpful discussions and contributions. Finally, we’d like to thank the data and infrastructure team at BAAI for their support on this project.

==> Bilingual CLIP draft/comment_management.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Comment management
\newcounter{lzCounter}
\newif\iflzvar
\lzvartrue
%\trvarfalse
\iflzvar
\newcommand{\luke}[1]{{\small \color{brown} \refstepcounter{lzCounter}\textsf{[LZ]$_{\arabic{lzCounter}}$:{#1}}}}
\else
\newcommand{\luca}[1]{}
\fi

\newcounter{srCounter}
\newif\ifsrvar
\srvartrue
%\trvarfalse
\ifsrvar
\newcommand{\seb}[1]{{\small \color{blue} \refstepcounter{srCounter}\textsf{[SR]$_{\arabic{srCounter}}$:{#1}}}}
\else
\newcommand{\seb}[1]{}
\fi

\newcounter{fpCounter}
\newif\iffpvar
\fpvartrue
%\trvarfalse
\iffpvar
\newcommand{\fabio}[1]{{\small \color{orange} \refstepcounter{fpCounter}\textsf{[FP]$_{\arabic{fpCounter}}$:{#1}}}}
\else
\newcommand{\fabio}[1]{}
\fi

\newcounter{lwCounter}
\newif\iflwvar
\lwvartrue
%\trvarfalse
\iflwvar
\newcommand{\ledell}[1]{{\small \color{purple} \refstepcounter{lwCounter}\textsf{[LW]$_{\arabic{lwCounter}}$:{#1}}}}
\else
\newcommand{\ledell}[1]{}
\fi

%\iftrue
\iffalse
\renewcommand{\luke}[1]{}
\renewcommand{\seb}[1]{}
\renewcommand{\fabio}[1]{}
\renewcommand{\ledell}[1]{}
\fi


==> Bilingual CLIP draft/figures/recall.tex <==
\begin{figure}[t]
    \centering
        \begin{tikzpicture}
        \begin{axis}[
            title={Top-$k$ entity retrieval accuracy},
            xlabel={$k$: number of retrieved entities},
            ylabel={Accuracy},
            xmin=0, xmax=200,
            ymin=0.15, ymax=1,
            xtick={1,50,100,150,200},
            ytick={0,0.2,0.4,0.6,0.8,1},
            legend pos=south east,
            ymajorgrids=true,
            grid style=dashed,
        ]
         
        \addplot[
            color=black,
            mark=square,
            mark size=1pt
            ]
            coordinates {
            (1, 0.2422)(5, 0.5322)(10, 0.6151)(30, 0.7191)(50, 0.7555)(70, 0.7796)(100, 0.8001)(200, 0.8324)(300, 0.8498)(400, 0.8596)(500, 0.8651)
            };
            \addlegendentry{BM25}

        \addplot[
            color=purple,
            mark=square,
            mark size=1pt
            ]
            coordinates {
            (1,0.4689)(5,0.7631)(10,0.8240)(30,0.8853)(50,0.9052)(70,0.9166)(100,0.9264)(200,0.9441)(300,0.9530) (400,0.9580) (500,0.9617)
            };
            \addlegendentry{Bi-encoder}


        \end{axis}
        \end{tikzpicture}
    \caption{Top-$k$ entity retrieval accuracy on validation dataset of Zero-shot EL dataset}
    \label{fig:retrieval}
\end{figure}


==> Bilingual CLIP draft/tables/table_classification.tex <==
\begin{table*}[thbp]
\small
\centering
\begin{tabular}{clccccc} 
\hline
\multirow{2}{*}{Language} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{5}{c}{Dataset}                                         \\ 
\cline{3-7}
                           & \multicolumn{1}{c}{}                         & Imagenet & ImageNet Sketch~ & ImageNet-A & ImageNet-R & ImageNetV2~  \\ 
\hline
\multirow{6}{*}{\rotatebox{90}{English}}   & CLIP                                         & \textbf{75.5}     & \textbf{59.6}             & \textbf{70.6}       & \textbf{87.9}       & \textbf{69.9}         \\
                           & M-CLIP                                       & 52.3     & 44.2             & 59.1       & 81.7       & 47.3         \\
                           %& M-CLIP$_B$                                      & 30       & 22.2             & 21.3       & 48.3       & 26.7         \\
                           & CN-CLIP                                      & 32.5     & 30.7             & 29.8       & 57         & 28.6         \\
                           & AltCLIP$_{T}$                                     & 74.7     & 59.2             & 70.4       & 87.9       & 68.8         \\
                           & AltCLIP                                      & 74.5     & 58.7             & 69.5       & 87.2       & 68.1         \\ 
\hline
\multirow{6}{*}{\rotatebox{90}{Chinese}}   & CLIP                                         & 1.9      & 1.9              & 6          & 5.3        & 1.8          \\
                           & M-CLIP                                       & 43       & 36.8             & 51.7       & 68.7       & 40.1         \\
                           %& M-CLIP$_B$                                      & 23.1     & 17.2             & 16.4       & 38.4       & 20.1         \\
                           & CN-CLIP                                      & 53.6     & \textbf{47.3}             & 43.1       & 77.6       & 48.3         \\
                           & AltCLIP$_{T}$                                     & 58.2     & 44.5             & 56.8       & 78         & 48.1         \\
                           & AltCLIP                                      & \textbf{59.6}     &46.5             & \textbf{58.5}       & \textbf{79.9}       &\textbf {50.9}         \\
\hline
\end{tabular}
\caption{Comparison Results of our proposed model and sota CLIP models on image classification benchmarks, i.e. ImageNet and its variants. AltCLIP$_{T}$ and AltCLIP are the same to Figure 2. All image encoders used in these models are Vit-L for fair comparison. The metric reported is zero-shot classification accuracy.}
\label{tab:imagenet}
\end{table*}

==> Bilingual CLIP draft/tables/table_retrieval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[hb]
\centering
\small
\begin{tabular}{ccccccccc}\hline
\multirow{2}{*}{Dataset}   & \multirow{2}{*}{Method} & \multicolumn{3}{l}{Text-to-Image Retrival} & \multicolumn{3}{l}{Image-to-Text Retrival} & \multirow{2}{*}{MR} \\\cline{3-8}
                           &                         & R@1          & R@5          & R@10         & R@1          & R@5          & R@10         &                     \\\hline
\multirow{7}{*}{\rotatebox{90}{Flickr30k$_{EN}$}} & CLIP         &    65.0          &     87.1         &      92.2        &    85.1          &      97.3        &    \textbf{99.2}          &  87.6                   \\
& Taiyi &25.3	&48.2	&59.2	&39.3	&68.1	&79.6	&53.3 \\ 
& Wukong &-	&-	&-	&-	&-	&-	&- \\
& R2D2 &-	&-	&-	&-	&-	&-	&-\\
& CN-CLIP & 49.5	&76.9	&83.8	&66.5	&91.2 	&96.0	&77.3 \\
& AltCLIP$_{T}$ &66.3	&87.8	&\textbf{92.7}	&85.9	&97.7	&99.1	&88.3 \\
& AltCLIP &\textbf{72.5}	&\textbf{91.6}	&\textbf{95.4}	&\textbf{86.0}	&\textbf{98.0}	&99.1 &	\textbf{90.4} 
               \\\hline
\multirow{7}{*}{\rotatebox{90}{Flickr30k$_{CN}$}} & CLIP         &       0      &      2.4        &     4.0         &     2.3         &   8.1           &     12.6        &    5.0                 \\
& Taiyi &53.7	&79.8	&86.6	&63.8	&90.5	&95.9	&78.4 \\
& Wukong$^{\dag}$ &51.7	&78.9	&86.3	&76.1	&94.8	&97.5	&80.9 \\
& R2D2$^{\dag}$ &60.9	&86.8	&92.7	&77.6	&96.7	&\textbf{98.9}	&85.6 \\
& CN-CLIP &68	&89.7	&94.4	&80.2	&96.6	&98.2	&87.9 \\
& AltCLIP$_{T}$&63.7	&86.3	&92.1	&84.7	&97.4	&98.7	&87.2 \\
& AltCLIP &\textbf{69.8}	&\textbf{89.9}	&\textbf{94.7}	&\textbf{84.8}	&\textbf{97.4}	&98.8	&\textbf{89.2}   
\\\hline

\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{EN}$}} & CLIP
               &36.5 &61.1  &71.1 &56.4 &79.5  &86.5  &65.2\\
&Taiyi &11.7 &27.8  &37.4 &19.8 &42.1  &54.3  &32.2 \\ 
&Wukong &-	&-	&-	&-	&-	&-	&- \\
&R2D2 &-	&-	&-	&-	&-	&-	&-\\
  
&CN-CLIP  &26.1 &50.0  &61.3 &40.9 &65.8  &76.3  &53.4\\
&AltCLIP$_{T}$&37.5 &62.1  &72.1 &57.2 &80.5  &87.5  &66.1  \\
&AltCLIP&\textbf{42.9} &\textbf{68.0}  &\textbf{77.4} &\textbf{58.6} &\textbf{80.6}  &\textbf{87.8}  &\textbf{69.2} 

               \\\hline
\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{CN}(1K)$}} & CLIP  &0.6 &4.1  &7.1 &1.8 &6.7  &11.9  &5.4 \\
&Taiyi&52.0 &80.2  &89.6 &46.6 &76.3  &88.6  &72.2  \\
&Wukong$^{\dag}$ &55.2& 81.0 &90.6 &53.4 &80.2 &90.1 &75.1 \\
&R2D2$^{\dag}$ &63.3 &\textbf{89.3} &\textbf{95.7} &56.4 &85.0 &93.1 &80.5 \\
&CN-CLIP &63.7 &88.7  &94.4 &61.0 &84.7  &93.6  &81.0 \\

&AltCLIP$_{T}$&55.7 &82.9  &91.2 &60.7 &86.3  &93.4  &78.4  \\
&AltCLIP&\textbf{63.9} &87.2  &93.9 &\textbf{62.8} &\textbf{88.8}  &\textbf{95.5}  &\textbf{82.0} 

\\\hline
\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{CN}(5K)$}} & CLIP  &0.8 &3.9  &5.8 &3.5 &8.9  &14.4  &6.2    \\
& Taiyi &46.1 &74.9  &85.1 &58.1 &83.9  &91.7  &73.3   \\
&Wukong &-	&-	&-	&-	&-	&-	&- \\
&R2D2&-	&-	&-	&-	&-	&-	&- \\
&CN-CLIP &58.6 &85.3  &92.7 &72.1 &90.9  &94.7  &82.4 \\
&AltCLIP$_{T}$ &54.9 &81.8  &90.5 &76.3 &93.9  &\textbf{97.6}  &82.5  \\
&AltCLIP&\textbf{61.3} &\textbf{86.0}  &\textbf{93.2} &\textbf{77.8} &\textbf{94.4}  &97.5  &\textbf{85.0} 
\\\hline
\end{tabular}
\caption{Experimental results on retrieval tasks, namely English and Chinese version of Flickr30k and MSCOCO. All image encoders used in these models are Vit-L for fair comparison. AltCLIP$_{T}$ denotes for our model after Teacher Learning stage while AltCLIP denotes for our model after contrastive learning stage.$^{\dag}$ represents we report original results from papers.}
\label{tab:retrieval}
\end{table*}

==> Bilingual CLIP draft/tables_backup/full_eval.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|cccccc}\hline                     
\multirow{2}{*}{Dataset}               & CLIP & Large  & Large & Large \\
& 400M & 28M & 36M & 2M \\\hline

Birdsnap                & \textbf{0.404}    & 0.311    & 0.357           & 0.320      \\
Caltech-101               & 0.868    & 0.872    & \textbf{0.881}           & 0.870      \\
Stanford Cars               & 0.778    & 0.736    & \textbf{0.781}           & 0.773      \\
CIFAR-10                     & \textbf{0.956}    & 0.948    & 0.952           & 0.954      \\
CIFAR-100                 & 0.758    & 0.779    & 0.757           & \textbf{0.789}      \\
Country211             & 0.317    & 0.269    & \textbf{0.318}           & 0.309      \\
DTD                    & 0.556    & \textbf{0.590}    & 0.577           & 0.566      \\
EuroSAT              & 0.624    & 0.643    & 0.657           & \textbf{0.669}      \\
Facial Emotion Recognition 2013                  & 0.499    & 0.544    & 0.558           & \textbf{0.563}      \\
FGVC Aircraft           & \textbf{0.320}    & 0.293    & 0.310           & 0.302      \\
Flickr30k            & 0.650    & 0.661    & 0.663           & \textbf{0.725}      \\
Oxford Flowers 102           & \textbf{0.792}    & 0.741    & 0.743           & 0.748      \\
Food-101                 & \textbf{0.931}    & 0.931    & 0.929           & 0.930      \\
GTSRB                  & 0.506    & 0.463    & \textbf{0.529}           & 0.511      \\
ImageNet Sketch       & \textbf{0.596}    & 0.592    & 0.592           & 0.587      \\
ImageNet               & \textbf{0.755}    & 0.744    & 0.747           & 0.745      \\
Imagenet-A                & \textbf{0.706}    & 0.695    & 0.704           & 0.695      \\
Imagenet-R          & \textbf{0.879}    & 0.872    & \textbf{0.879}           & 0.872      \\
ImageNetV2              & \textbf{0.699}    & 0.680    & 0.688           & 0.681      \\
Kinetics400            & 0.529    & \textbf{0.533}    & 0.523           & 0.526      \\
Kinetics600          & 0.524    & \textbf{0.529}    & 0.525           & 0.522      \\
MNIST                  & \textbf{0.763}    & 0.655    & 0.737           & 0.691      \\
MSCOCO & 0.356     & 0.373    & 0.375           & \textbf{0.429}      \\
ObjectNet              & 0.690    & 0.685    & \textbf{0.696}           & 0.689      \\
PatchCamelyon                      & 0.520    & 0.490    & \textbf{0.655}           & 0.577      \\
Oxford-IIIT Pets              & 0.935    & 0.928    & 0.931           & \textbf{0.936}      \\
Rendered SST2            & 0.690    & 0.689    & 0.691           & \textbf{0.724}      \\
RESISC45              & 0.647    & \textbf{0.691}    & 0.656           & 0.665      \\
STL-10                 & 0.994    & 0.994    & 0.994           & 0.994      \\
SUN397                & 0.676    & \textbf{0.697}    & 0.676           & 0.695      \\
UCF101                  & \textbf{0.764}    & 0.760    & 0.753           & 0.756      \\
Pascal VOC 2007 Classification                  & 0.782    & 0.770    & 0.798           & \textbf{0.814}      \\
Pascal VOC 2007 Multilabel Classification           & 0.790    & 0.825    & 0.799           & \textbf{0.814}      \\\hline
\end{tabular}
\caption{Results on CLIP benchmark.\label{tab:ccl}}
\end{table*}


==> comment_management.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Comment management
\newcounter{lzCounter}
\newif\iflzvar
\lzvartrue
%\trvarfalse
\iflzvar
\newcommand{\luke}[1]{{\small \color{brown} \refstepcounter{lzCounter}\textsf{[LZ]$_{\arabic{lzCounter}}$:{#1}}}}
\else
\newcommand{\luca}[1]{}
\fi

\newcounter{srCounter}
\newif\ifsrvar
\srvartrue
%\trvarfalse
\ifsrvar
\newcommand{\seb}[1]{{\small \color{blue} \refstepcounter{srCounter}\textsf{[SR]$_{\arabic{srCounter}}$:{#1}}}}
\else
\newcommand{\seb}[1]{}
\fi

\newcounter{fpCounter}
\newif\iffpvar
\fpvartrue
%\trvarfalse
\iffpvar
\newcommand{\fabio}[1]{{\small \color{orange} \refstepcounter{fpCounter}\textsf{[FP]$_{\arabic{fpCounter}}$:{#1}}}}
\else
\newcommand{\fabio}[1]{}
\fi

\newcounter{lwCounter}
\newif\iflwvar
\lwvartrue
%\trvarfalse
\iflwvar
\newcommand{\ledell}[1]{{\small \color{purple} \refstepcounter{lwCounter}\textsf{[LW]$_{\arabic{lwCounter}}$:{#1}}}}
\else
\newcommand{\ledell}[1]{}
\fi

%\iftrue
\iffalse
\renewcommand{\luke}[1]{}
\renewcommand{\seb}[1]{}
\renewcommand{\fabio}[1]{}
\renewcommand{\ledell}[1]{}
\fi


==> figures/recall.tex <==
\begin{figure}[t]
    \centering
        \begin{tikzpicture}
        \begin{axis}[
            title={Top-$k$ entity retrieval accuracy},
            xlabel={$k$: number of retrieved entities},
            ylabel={Accuracy},
            xmin=0, xmax=200,
            ymin=0.15, ymax=1,
            xtick={1,50,100,150,200},
            ytick={0,0.2,0.4,0.6,0.8,1},
            legend pos=south east,
            ymajorgrids=true,
            grid style=dashed,
        ]
         
        \addplot[
            color=black,
            mark=square,
            mark size=1pt
            ]
            coordinates {
            (1, 0.2422)(5, 0.5322)(10, 0.6151)(30, 0.7191)(50, 0.7555)(70, 0.7796)(100, 0.8001)(200, 0.8324)(300, 0.8498)(400, 0.8596)(500, 0.8651)
            };
            \addlegendentry{BM25}

        \addplot[
            color=purple,
            mark=square,
            mark size=1pt
            ]
            coordinates {
            (1,0.4689)(5,0.7631)(10,0.8240)(30,0.8853)(50,0.9052)(70,0.9166)(100,0.9264)(200,0.9441)(300,0.9530) (400,0.9580) (500,0.9617)
            };
            \addlegendentry{Bi-encoder}


        \end{axis}
        \end{tikzpicture}
    \caption{Top-$k$ entity retrieval accuracy on validation dataset of Zero-shot EL dataset}
    \label{fig:retrieval}
\end{figure}


==> tables/table_classification.tex <==
\begin{table*}[thbp]
\small
\centering
\begin{tabular}{clccccc} 
\hline
\multirow{2}{*}{Language} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{5}{c}{Dataset}                                         \\ 
\cline{3-7}
                           & \multicolumn{1}{c}{}                         & Imagenet & ImageNet Sketch~ & ImageNet-A & ImageNet-R & ImageNetV2~  \\ 
\hline
\multirow{6}{*}{\rotatebox{90}{English}}   & CLIP                                         & \textbf{75.5}     & \textbf{59.6}             & \textbf{70.6}       & \textbf{87.9}       & \textbf{69.9}         \\
                           & M-CLIP                                       & 52.3     & 44.2             & 59.1       & 81.7       & 47.3         \\
                           %& M-CLIP$_B$                                      & 30       & 22.2             & 21.3       & 48.3       & 26.7         \\
                           & CN-CLIP                                      & 32.5     & 30.7             & 29.8       & 57         & 28.6         \\
                           & AltCLIP$_{T}$                                     & 74.7     & 59.2             & 70.4       & 87.9       & 68.8         \\
                           & AltCLIP                                      & 74.5     & 58.7             & 69.5       & 87.2       & 68.1         \\ 
\hline
\multirow{6}{*}{\rotatebox{90}{Chinese}}   & CLIP                                         & 1.9      & 1.9              & 6          & 5.3        & 1.8          \\
                           & M-CLIP                                       & 43       & 36.8             & 51.7       & 68.7       & 40.1         \\
                           %& M-CLIP$_B$                                      & 23.1     & 17.2             & 16.4       & 38.4       & 20.1         \\
                           & CN-CLIP                                      & 53.6     & \textbf{47.3}             & 43.1       & 77.6       & 48.3         \\
                           & AltCLIP$_{T}$                                     & 58.2     & 44.5             & 56.8       & 78         & 48.1         \\
                           & AltCLIP                                      & \textbf{59.6}     &46.5             & \textbf{58.5}       & \textbf{79.9}       &\textbf {50.9}         \\
\hline
\end{tabular}
\caption{Comparison Results of our proposed model and sota CLIP models on image classification benchmarks, i.e. ImageNet and its variants. AltCLIP$_{T}$ and AltCLIP are the same to Figure 2. All image encoders used in these models are Vit-L for fair comparison. The metric reported is zero-shot classification accuracy.}
\label{tab:imagenet}
\end{table*}

==> tables/table_retrieval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[hb]
\centering
\small
\begin{tabular}{ccccccccc}\hline
\multirow{2}{*}{Dataset}   & \multirow{2}{*}{Method} & \multicolumn{3}{l}{Text-to-Image Retrival} & \multicolumn{3}{l}{Image-to-Text Retrival} & \multirow{2}{*}{MR} \\\cline{3-8}
                           &                         & R@1          & R@5          & R@10         & R@1          & R@5          & R@10         &                     \\\hline
\multirow{7}{*}{\rotatebox{90}{Flickr30k$_{EN}$}} & CLIP         &    65.0          &     87.1         &      92.2        &    85.1          &      97.3        &    \textbf{99.2}          &  87.6                   \\
& Taiyi &25.3	&48.2	&59.2	&39.3	&68.1	&79.6	&53.3 \\ 
& Wukong &-	&-	&-	&-	&-	&-	&- \\
& R2D2 &-	&-	&-	&-	&-	&-	&-\\
& CN-CLIP & 49.5	&76.9	&83.8	&66.5	&91.2 	&96.0	&77.3 \\
& AltCLIP$_{T}$ &66.3	&87.8	&\textbf{92.7}	&85.9	&97.7	&99.1	&88.3 \\
& AltCLIP &\textbf{72.5}	&\textbf{91.6}	&\textbf{95.4}	&\textbf{86.0}	&\textbf{98.0}	&99.1 &	\textbf{90.4} 
               \\\hline
\multirow{7}{*}{\rotatebox{90}{Flickr30k$_{CN}$}} & CLIP         &       0      &      2.4        &     4.0         &     2.3         &   8.1           &     12.6        &    5.0                 \\
& Taiyi &53.7	&79.8	&86.6	&63.8	&90.5	&95.9	&78.4 \\
& Wukong$^{\dag}$ &51.7	&78.9	&86.3	&76.1	&94.8	&97.5	&80.9 \\
& R2D2$^{\dag}$ &60.9	&86.8	&92.7	&77.6	&96.7	&\textbf{98.9}	&85.6 \\
& CN-CLIP &68	&89.7	&94.4	&80.2	&96.6	&98.2	&87.9 \\
& AltCLIP$_{T}$&63.7	&86.3	&92.1	&84.7	&97.4	&98.7	&87.2 \\
& AltCLIP &\textbf{69.8}	&\textbf{89.9}	&\textbf{94.7}	&\textbf{84.8}	&\textbf{97.4}	&98.8	&\textbf{89.2}   
\\\hline

\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{EN}$}} & CLIP
               &36.5 &61.1  &71.1 &56.4 &79.5  &86.5  &65.2\\
&Taiyi &11.7 &27.8  &37.4 &19.8 &42.1  &54.3  &32.2 \\ 
&Wukong &-	&-	&-	&-	&-	&-	&- \\
&R2D2 &-	&-	&-	&-	&-	&-	&-\\
  
&CN-CLIP  &26.1 &50.0  &61.3 &40.9 &65.8  &76.3  &53.4\\
&AltCLIP$_{T}$&37.5 &62.1  &72.1 &57.2 &80.5  &87.5  &66.1  \\
&AltCLIP&\textbf{42.9} &\textbf{68.0}  &\textbf{77.4} &\textbf{58.6} &\textbf{80.6}  &\textbf{87.8}  &\textbf{69.2} 

               \\\hline
\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{CN}(1K)$}} & CLIP  &0.6 &4.1  &7.1 &1.8 &6.7  &11.9  &5.4 \\
&Taiyi&52.0 &80.2  &89.6 &46.6 &76.3  &88.6  &72.2  \\
&Wukong$^{\dag}$ &55.2& 81.0 &90.6 &53.4 &80.2 &90.1 &75.1 \\
&R2D2$^{\dag}$ &63.3 &\textbf{89.3} &\textbf{95.7} &56.4 &85.0 &93.1 &80.5 \\
&CN-CLIP &63.7 &88.7  &94.4 &61.0 &84.7  &93.6  &81.0 \\

&AltCLIP$_{T}$&55.7 &82.9  &91.2 &60.7 &86.3  &93.4  &78.4  \\
&AltCLIP&\textbf{63.9} &87.2  &93.9 &\textbf{62.8} &\textbf{88.8}  &\textbf{95.5}  &\textbf{82.0} 

\\\hline
\multirow{7}{*}{\rotatebox{90}{MSCOCO$_{CN}(5K)$}} & CLIP  &0.8 &3.9  &5.8 &3.5 &8.9  &14.4  &6.2    \\
& Taiyi &46.1 &74.9  &85.1 &58.1 &83.9  &91.7  &73.3   \\
&Wukong &-	&-	&-	&-	&-	&-	&- \\
&R2D2&-	&-	&-	&-	&-	&-	&- \\
&CN-CLIP &58.6 &85.3  &92.7 &72.1 &90.9  &94.7  &82.4 \\
&AltCLIP$_{T}$ &54.9 &81.8  &90.5 &76.3 &93.9  &\textbf{97.6}  &82.5  \\
&AltCLIP&\textbf{61.3} &\textbf{86.0}  &\textbf{93.2} &\textbf{77.8} &\textbf{94.4}  &97.5  &\textbf{85.0} 
\\\hline
\end{tabular}
\caption{Experimental results on retrieval tasks, namely English and Chinese version of Flickr30k and MSCOCO. All image encoders used in these models are Vit-L for fair comparison. AltCLIP$_{T}$ denotes for our model after Teacher Learning stage while AltCLIP denotes for our model after contrastive learning stage.$^{\dag}$ represents we report original results from papers.}
\label{tab:retrieval}
\end{table*}

==> tables_backup/full_eval.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|cccccc}\hline                     
\multirow{2}{*}{Dataset}               & CLIP & Large  & Large & Large \\
& 400M & 28M & 36M & 2M \\\hline

Birdsnap                & \textbf{0.404}    & 0.311    & 0.357           & 0.320      \\
Caltech-101               & 0.868    & 0.872    & \textbf{0.881}           & 0.870      \\
Stanford Cars               & 0.778    & 0.736    & \textbf{0.781}           & 0.773      \\
CIFAR-10                     & \textbf{0.956}    & 0.948    & 0.952           & 0.954      \\
CIFAR-100                 & 0.758    & 0.779    & 0.757           & \textbf{0.789}      \\
Country211             & 0.317    & 0.269    & \textbf{0.318}           & 0.309      \\
DTD                    & 0.556    & \textbf{0.590}    & 0.577           & 0.566      \\
EuroSAT              & 0.624    & 0.643    & 0.657           & \textbf{0.669}      \\
Facial Emotion Recognition 2013                  & 0.499    & 0.544    & 0.558           & \textbf{0.563}      \\
FGVC Aircraft           & \textbf{0.320}    & 0.293    & 0.310           & 0.302      \\
Flickr30k            & 0.650    & 0.661    & 0.663           & \textbf{0.725}      \\
Oxford Flowers 102           & \textbf{0.792}    & 0.741    & 0.743           & 0.748      \\
Food-101                 & \textbf{0.931}    & 0.931    & 0.929           & 0.930      \\
GTSRB                  & 0.506    & 0.463    & \textbf{0.529}           & 0.511      \\
ImageNet Sketch       & \textbf{0.596}    & 0.592    & 0.592           & 0.587      \\
ImageNet               & \textbf{0.755}    & 0.744    & 0.747           & 0.745      \\
Imagenet-A                & \textbf{0.706}    & 0.695    & 0.704           & 0.695      \\
Imagenet-R          & \textbf{0.879}    & 0.872    & \textbf{0.879}           & 0.872      \\
ImageNetV2              & \textbf{0.699}    & 0.680    & 0.688           & 0.681      \\
Kinetics400            & 0.529    & \textbf{0.533}    & 0.523           & 0.526      \\
Kinetics600          & 0.524    & \textbf{0.529}    & 0.525           & 0.522      \\
MNIST                  & \textbf{0.763}    & 0.655    & 0.737           & 0.691      \\
MSCOCO & 0.356     & 0.373    & 0.375           & \textbf{0.429}      \\
ObjectNet              & 0.690    & 0.685    & \textbf{0.696}           & 0.689      \\
PatchCamelyon                      & 0.520    & 0.490    & \textbf{0.655}           & 0.577      \\
Oxford-IIIT Pets              & 0.935    & 0.928    & 0.931           & \textbf{0.936}      \\
Rendered SST2            & 0.690    & 0.689    & 0.691           & \textbf{0.724}      \\
RESISC45              & 0.647    & \textbf{0.691}    & 0.656           & 0.665      \\
STL-10                 & 0.994    & 0.994    & 0.994           & 0.994      \\
SUN397                & 0.676    & \textbf{0.697}    & 0.676           & 0.695      \\
UCF101                  & \textbf{0.764}    & 0.760    & 0.753           & 0.756      \\
Pascal VOC 2007 Classification                  & 0.782    & 0.770    & 0.798           & \textbf{0.814}      \\
Pascal VOC 2007 Multilabel Classification           & 0.790    & 0.825    & 0.799           & \textbf{0.814}      \\\hline
\end{tabular}
\caption{Results on CLIP benchmark.\label{tab:ccl}}
\end{table*}

